Topological AdS/CFT and the $\Omega$ deformation

In this note, we define a holographic dual to four-dimensional superconformal field theories formulated on arbitrary Riemannian manifolds equipped with a Killing vector. Moreover, assuming smoothness of the bulk solution, we study the variation of the holographically renormalized supergravity action in the class of metrics on the boundary four-manifold with a prescribed isometry.

==> OmegaDeformationFiles/titlepage.tex <==
\title{Omega deformation and gravity dual}

%\preprint{preprint code}

\author[a]{Pietro Benetti Genolini,}
\author[b]{Paul Richmond}

\affiliation[a]{Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Wilberforce Road, Cambridge, CB3 OWA, UK}
\affiliation[b]{Department of Mathematics, King's College London, Strand, WC2R 2LS, UK}

\emailAdd{Pietro.BenettiGenolini@damtp.cam.ac.uk}
\emailAdd{Paul.Richmond@kcl.ac.uk}

\abstract{
some abstract}

%\keywords{}

\renewcommand{\baselinestretch}{1.05}
